LLMs in the Heart of Differential Testing: A Case Study on a Medical Rule Engine

The Cancer Registry of Norway (CRN) uses an automated cancer registration support system (CaReSS) to support core cancer registry activities, i.e, data capture, data curation, and producing data products and statistics for various stakeholders. GURI is a core component of CaReSS, which is responsible for validating incoming data with medical rules. Such medical rules are manually implemented by medical experts based on medical standards, regulations, and research. Since large language models (LLMs) have been trained on a large amount of public information, including these documents, they can be employed to generate tests for GURI. Thus, we propose an LLM-based test generation and differential testing approach (LLMeDiff) to test GURI. We experimented with four different LLMs, two medical rule engine implementations, and 58 real medical rules to investigate the hallucination, success, time efficiency, and robustness of the LLMs to generate tests, and these tests' ability to find potential issues in GURI. Our results showed that GPT-3.5 hallucinates the least, is the most successful, and is generally the most robust; however, it has the worst time efficiency. Our differential testing revealed 22 medical rules where implementation inconsistencies were discovered (e.g., regarding handling rule versions). Finally, we provide insights for practitioners and researchers based on the results.

==> metrics_table.tex <==
\begin{table*}[tbp]
    \footnotesize
    \centering
    \caption{\glspl{rq}, Objectives, Evaluation Metrics, and Statistical Tests}
    \label{tab:my-table}
      % \resizebox{\textwidth}{!}{%
    \begin{tabular}{llll}
        \toprule
        \textbf{RQ\#} & \textbf{Study Objective} & \textbf{Evaluation Metrics} & \textbf{Statistical Tests} \\ 
        \midrule
        1.1 & Hallucination & $CR_{overall}$, $CR_{complexity}$ & \\ 
        1.2 & Effectiveness & $SI_{overall}$, $SI_{testtype}$, $SI_{overall/testtype}$, $S_{overall/complexity}$, $SI_{testtype/complexity}$ & \\ 
        1.3 & Time cost & $time_{inference}$ & \\ \midrule
        2.1 & Robustness by test type & $R_{overall}$, $R_{testtype}$, $R_{overall/complexity}$, $R_{testtype/complexity}$ & \\ 
        2.2 & Robustness by mutation type& $R_{mutationtype}$, $R_{mutationtype/complexity}$ & \\ \midrule
        3.1 & Result matches with GURI & $Match_{testtype/overall}$ & \\ 
        3.2 & Result mismatches with GURI & $Mismatch_{testtype/testtype\_pair}$ & \\ 
        \bottomrule
    \end{tabular}%
    % }
\end{table*}


==> rq2_table_mutation_operators.tex <==
\begin{table*}[htbp]
    \footnotesize
  \centering
  \caption{Median robustness indices per mutation operator, test type, and \gls{llm}}
  \label{tab:rq2:mutation:means}
  % \resizebox{\textwidth}{!}{%
  \input{rq2_table_mutation_operators_body.tex}
% }
\end{table*}

==> rq2_table_mutation_operators_body.tex <==
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
Mut. & \multicolumn{4}{c}{\metricRIPass{}} & \multicolumn{4}{c}{\metricRIFail{}} & \multicolumn{4}{c}{\metricRINA{}} \\
\cmidrule(l{1pt}r{1pt}){2-5}
\cmidrule(l{1pt}r{1pt}){6-9}
\cmidrule(l{1pt}r{1pt}){10-13}
& \mistral{} & \llama{} & \mixtral{} & \gpt{} & \mistral{} & \llama{} & \mixtral{} & \gpt{} & \mistral{} & \llama{} & \mixtral{} & \gpt{} \\
\midrule

\mutACO{} & \perc{95.53} & \perc{99.96} & \perc{95.55} & \perc{99.69} & \perc{95.53} & \perc{98.62} & \perc{89.1} & \perc{96.78} & \perc{93.4} & \perc{92.64} & \perc{91.47} & \perc{93.33} \\
\mutAD{} & \perc{93.29} & \perc{100} & \perc{98.43} & \perc{99.72} & \perc{85.995} & \perc{100} & \perc{95} & \perc{96.545} & \perc{90.995} & \perc{90.57} & \perc{93.485} & \perc{96.34} \\
\mutCO{} & \perc{87.59} & \perc{92.86} & \perc{85.77} & \perc{93.27} & \perc{90.175} & \perc{82.845} & \perc{86.6} & \perc{84.675} & \perc{91.905} & \perc{87.52} & \perc{90.03} & \perc{90.57} \\
\mutNI{} & \perc{84.565} & \perc{95.345} & \perc{90} & \perc{97.64} & \perc{88.74} & \perc{85.165} & \perc{86.43} & \perc{74.07} & \perc{89.485} & \perc{86.39} & \perc{90.735} & \perc{97.365} \\
\mutRI{} & \perc{89.32} & \perc{95.27} & \perc{91.41} & \perc{97.64} & \perc{89.75} & \perc{89.99} & \perc{92.83} & \perc{88.22} & \perc{87.48} & \perc{85.86} & \perc{93.05} & \perc{96.67} \\
\mutRSE{} & \perc{92.2} & \perc{83.8} & \perc{84.98} & \perc{100} & \perc{96.27} & \perc{97.65} & \perc{91.72} & \perc{92.93} & \perc{88.76} & \perc{95.2} & \perc{88.75} & \perc{95.29} \\
\mutSR{} & \perc{93.34} & \perc{95.04} & \perc{88.31} & \perc{97.64} & \perc{87.3} & \perc{77.01} & \perc{80.01} & \perc{78.78} & \perc{86.67} & \perc{76.43} & \perc{86.67} & \perc{97.64} \\
\mutSSI{} & \perc{94.385} & \perc{96.665} & \perc{93.275} & \perc{94.86} & \perc{95.975} & \perc{97.64} & \perc{90.73} & \perc{89.67} & \perc{93.185} & \perc{93.265} & \perc{90.715} & \perc{97.155} \\
\midrule
Overall & \perc{89.6} & \perc{94.82} & \perc{89.88} & \perc{97.64} & \perc{90.175} & \perc{88.325} & \perc{88.31} & \perc{85.86} & \perc{89.665} & \perc{87.14} & \perc{90.62} & \perc{96.67} \\

\bottomrule
\end{tabular}


==> rq2_table_stats_mutation_operators.tex <==
\begin{table}[tbp]
    \centering
    \scriptsize
    \caption{Pair-wise statistical tests of the robustness indices per mutation operator, test type, and \gls{llm} (only differences)}
    \label{tab:rq2:stats:mutation_types}
    \resizebox{\columnwidth}{!}{%
    \input{rq2_table_stats_mutation_operators_body.tex}
    }
\end{table}

==> rq2_table_stats_mutation_operators_body.tex <==
\begin{tabular}{lllllrrl}
\toprule
Mut. & Metric & Model 1 & Model 2 & Comp. & \pvalue{} & \vda{} & Magnitude \\
\midrule

\mutAD{} & \metricRIPass{} & \mistral{} & \llama{} & \statWorse{} & \pval{0.000889} & \vdaval{0} & large \\
\midrule{}
\mutNI{} & \metricRIPass{} & \mistral{} & \llama{} & \statWorse{} & \pval{0.00122} & \vdaval{0.363} & small \\
 &  & \mistral{} & \gpt{} & \statWorse{} & \pval{1.18e-11} & \vdaval{0.207} & large \\
 &  & \llama{} & \gpt{} & \statWorse{} & \pval{0.00173} & \vdaval{0.369} & small \\
 &  & \mixtral{} & \gpt{} & \statWorse{} & \pval{7.9e-08} & \vdaval{0.242} & large \\
\cmidrule(l{1pt}r{1pt}){2-8}
 & \metricRIFail{} & \mistral{} & \gpt{} & \statBetter{} & \pval{0.0047} & \vdaval{0.645} & small \\
\cmidrule(l{1pt}r{1pt}){2-8}
 & \metricRINA{} & \mistral{} & \gpt{} & \statWorse{} & \pval{0.0011} & \vdaval{0.348} & small \\
 &  & \llama{} & \gpt{} & \statWorse{} & \pval{2.64e-05} & \vdaval{0.317} & medium \\
\midrule{}
\mutRI{} & \metricRIPass{} & \mistral{} & \gpt{} & \statWorse{} & \pval{6.74e-07} & \vdaval{0.219} & large \\
 &  & \mixtral{} & \gpt{} & \statWorse{} & \pval{0.000502} & \vdaval{0.291} & medium \\
\cmidrule(l{1pt}r{1pt}){2-8}
 & \metricRINA{} & \llama{} & \gpt{} & \statWorse{} & \pval{0.000131} & \vdaval{0.3} & medium \\
\midrule{}
\mutRSE{} & \metricRIPass{} & \llama{} & \gpt{} & \statWorse{} & \pval{0.00294} & \vdaval{0.149} & large \\
 &  & \mixtral{} & \gpt{} & \statWorse{} & \pval{0.00024} & \vdaval{0.0756} & large \\
\midrule{}
\mutSR{} & \metricRIPass{} & \mistral{} & \gpt{} & \statWorse{} & \pval{0.00036} & \vdaval{0.238} & large \\
 &  & \mixtral{} & \gpt{} & \statWorse{} & \pval{5.83e-06} & \vdaval{0.197} & large \\
\cmidrule(l{1pt}r{1pt}){2-8}
 & \metricRINA{} & \llama{} & \gpt{} & \statWorse{} & \pval{6.78e-05} & \vdaval{0.268} & medium \\
\midrule{}
Overall & \metricRIPass{} & \mistral{} & \llama{} & \statWorse{} & \pval{4.37e-05} & \vdaval{0.407} & small \\
 &  & \mistral{} & \gpt{} & \statWorse{} & \pval{4.67e-21} & \vdaval{0.27} & medium \\
 &  & \llama{} & \mixtral{} & \statBetter{} & \pval{0.000284} & \vdaval{0.581} & small \\
 &  & \llama{} & \gpt{} & \statWorse{} & \pval{5.22e-07} & \vdaval{0.393} & small \\
 &  & \mixtral{} & \gpt{} & \statWorse{} & \pval{2.31e-19} & \vdaval{0.286} & medium \\
\cmidrule(l{1pt}r{1pt}){2-8}
 & \metricRIFail{} & \mistral{} & \gpt{} & \statBetter{} & \pval{0.000106} & \vdaval{0.605} & small \\
\cmidrule(l{1pt}r{1pt}){2-8}
 & \metricRINA{} & \mistral{} & \gpt{} & \statWorse{} & \pval{3.54e-07} & \vdaval{0.368} & small \\
 &  & \llama{} & \mixtral{} & \statWorse{} & \pval{0.00509} & \vdaval{0.416} & small \\
 &  & \llama{} & \gpt{} & \statWorse{} & \pval{2.2e-15} & \vdaval{0.329} & medium \\
 &  & \mixtral{} & \gpt{} & \statWorse{} & \pval{2.06e-06} & \vdaval{0.368} & small \\

\bottomrule
\end{tabular}

